BioMedLM: A 2.7B Parameter Language Model Trained On Biomedical Text

Models such as GPT-4 and Med-PaLM 2 have demonstrated impressive performance on a wide variety of biomedical NLP tasks. However, these models have hundreds of billions of parameters, are computationally expensive to run, require users to send their input data over the internet, and are trained on unknown data sources. Can smaller, more targeted models compete? To address this question, we build and release BioMedLM, a 2.7 billion parameter GPT-style autoregressive model trained exclusively on PubMed abstracts and full articles. When fine-tuned, BioMedLM can produce strong multiple-choice biomedical question-answering results competitive with much larger models, such as achieving a score of 57.3% on MedMCQA (dev) and 69.0% on the MMLU Medical Genetics exam. BioMedLM can also be fine-tuned to produce useful answers to patient questions on medical topics. This demonstrates that smaller models can potentially serve as transparent, privacy-preserving, economical and environmentally friendly foundations for particular NLP applications, such as in biomedicine. The model is available on the Hugging Face Hub: https://huggingface.co/stanford-crfm/BioMedLM.

==> consumerqa.tex <==
\textbf{Question}

What does vitamin D do?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
Vitamin D plays an important role in maintaining your bones and supporting your immune system. It's also involved in many other body processes.

Vitamin D is a fat-soluble vitamin. Your body needs to get this vitamin from your diet and/or your sun exposure. You can get vitamin D from foods that contain vitamin D, such as fatty fish, eggs and fortified milk. You can also get vitamin D from sun exposure. 

Your body needs to get enough vitamin D to function properly. Vitamin D deficiency can cause rickets in children and osteomalacia in adults. Vitamin D deficiency can also cause muscle weakness and an increased risk of falls and bone fractures.

Vitamin D deficiency is a common condition. In the United States, about 1 in 10 people have vitamin D deficiency.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

What are good treatments for arthritis?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
There are many treatments for arthritis. Your healthcare provider will recommend the treatment that's right for you based on your symptoms and the type of arthritis you have. Treatments for arthritis include:

Medications: Your healthcare provider may prescribe medications to reduce pain and inflammation. Common medications include:

Nonsteroidal anti-inflammatory drugs (NSAIDs).

Corticosteroids.

Pain relievers.

Physical therapy: Physical therapy can help you manage arthritis symptoms. Your healthcare provider may recommend exercises to strengthen muscles and improve flexibility.
Surgery: You may need surgery if your arthritis is severe or you don't respond to other treatments. Your healthcare provider may recommend joint replacement surgery or osteotomy.

Complications of arthritis treatments
You may experience side effects from arthritis treatments. Your healthcare provider will discuss the benefits and risks of your treatment options with you.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

What are the common causes of lower back pain?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
The most common causes of lower back pain include:

Degenerative disk disease: Damage to the disks in your lower back causes your disks to wear down. This wear and tear can lead to lower back pain.

Spinal stenosis: A narrowing of your spinal canal can cause pressure on your nerves and lower back pain.

Scoliosis: A curved spine can cause pain in your lower back.

Herniated disk: A bulge in one of your disks causes pain.

Spinal infection: Infections in your spine can cause pain and other symptoms.

Pregnancy: Your body is more sensitive during pregnancy, which can cause back pain.

Trauma: A fall, car accident or other injury can cause pain in your lower back.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

What are the best ways to unclog your ears?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
There are several ways to unclog your ears. Your healthcare provider will recommend the method that's right for you.

Ear drops: Your healthcare provider will apply ear drops to your ears. The drops may contain a steroid or antibiotic.

Ear tubes: Your healthcare provider will surgically insert a small tube into your ear canal. The tube drains fluid and helps drain ear infections.

Surgery: Your healthcare provider may perform ear surgery to remove excess ear tissue or open up your ear canal.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

How do you know if ear pain is serious?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
Ear pain can be a symptom of a serious health condition. If you have ear pain that lasts longer than a few days, or if it gets worse or doesn't go away, you should contact your healthcare provider.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

What do night sweats indicate?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
Night sweats are a symptom of many different conditions. If you have night sweats, it's important to talk to a healthcare provider about what's causing them.

\\~\\
\hrule
\\~\\
\\~\\

\textbf{Question}

How serious is hepatitis A?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
Hepatitis A is usually mild and doesn't cause long-term health problems. Most people recover fully from the infection without any medical treatment.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

How can I stop diarrhea?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
The best way to stop diarrhea is to treat the cause. If you have an infection, your healthcare provider may prescribe antibiotics. If you have a food poisoning outbreak, you can go to the emergency room or call your healthcare provider to get help. If you have chronic diarrhea, you may need to change your diet. If you have an autoimmune disease, your healthcare provider may prescribe medication. If you take a medication that causes diarrhea, you may need to stop taking it.

\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

What happens if listeria is left untreated?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
Listeria can cause serious illness and death if it's not treated. Up to 30\% of people with listeriosis die from the infection.
\\~\\
\hrule

\\~\\
\\~\\

\textbf{Question}

\\~\\
Does stress cause nosebleed?

\\~\\
\textbf{BioMedLM Answer}
\\~\\
Yes. Stress, anxiety and panic can increase your heart rate and blood pressure, which can lead to nosebleeds.

\\~\\
\hrule

\\~\\

\\~\\

==> qa.tex <==
\hypertarget{medmcqa}{\section{MedMCQA 
Example Questions}}
\label{app:medmcqa}

\\~\\
\hrule

\\~\\
\\~\\
\textbf{Question}

\\~\\
All of the following statements are true regarding hypertrophy, except:

\\~\\
A) Occurs due to synthesis and assembly of additional intracellular components.

\noindent B) There is an increase in the size of the cells.

\noindent C) Cells capable of division respond to stress by hypertrophy and hyperplasia.

\noindent \textbf{D) There is an increase in the number of cells.}
\\~\\

\\~\\
\textbf{Question}

\\~\\
A 19 year old female presents with pain in the neck for 5 days. She is not able to wear tie for her job because of neck pain. H\/O fatigue and lethargy for 10 days. She had flu like symptoms 20 days ago which resolved spontaneously. BP 110\/80 mmHg, Pulse 48\/min. Extremities are cold and dry. Neck is very tender. ECG normal. TSH is elevated. ESR 30 mm\/hr. Next appropriate step

\\~\\
A) Atropine injection

\noindent B) Levothyroxine administration

\noindent \textbf{C) Aspirin}

\noindent D) Increase iodine intake in food
\\~\\

\hrule

\hypertarget{medqa}{\section{MedQA Example Questions}}
\label{app:medqa}

\\~\\
\hrule

\\~\\
\\~\\
\textbf{Question}

\\~\\
A 45-year-old woman presents to the emergency department with acute onset of severe right upper quadrant abdominal pain that radiates to the infrascapular region. Her medical history is significant for obesity, hypertension, obstructive sleep apnea, and gastric bypass surgery 2 years ago after which she lost 79 kg (150 lb). The patient complains of nausea and vomiting that accompanies the pain. Her temperature is 38.9°C (101.2°F), blood pressure is 144/88 mm Hg, heart rate is 76/min, and respiratory rate is 14/min (fever). Abdominal examination is significant for right upper quadrant tenderness along with guarding and cessation of inspired breath on deep palpation of the right upper quadrant. Which test should be ordered first for this patient?

\\~\\
\textbf{A) Abdominal ultrasound}

\noindent B) CT scan of the abdomen

\noindent C) MRI of the abdomen

\noindent D) X-ray film of the abdomen
\\~\\
\hrule

\\~\\

\hypertarget{mmlu}{\section{MMLU Example Question}}
\label{app:mmlu}

\\~\\
\hrule

\\~\\
\\~\\
\textbf{Question}

\\~\\
Zinc finger proteins and helix-turn-helix proteins are

\\~\\
\textbf{A) types of DNA-binding proteins}

\noindent B) involved in the control of translation

\noindent C) components of ribosomes

\noindent D) part of the hemoglobin in blood cells
\\~\\
\hrule

\\~\\

\hypertarget{pubmedqa}{\section{PubMedQA Example Question}}
\label{app:pubmedqa}

\\~\\
\\~\\
\hrule

\\~\\
\\~\\
\textbf{Context}

\\~\\
To evaluate the degree to which histologic chorioamnionitis, a frequent finding in placentas submitted for histopathologic evaluation, correlates with clinical indicators of infection in the mother. A retrospective review was performed on 52 cases with a histologic diagnosis of acute chorioamnionitis from 2,051 deliveries at University Hospital, Newark, from January 2003 to July 2003. Third-trimester placentas without histologic chorioamnionitis (n = 52) served as controls. Cases and controls were selected sequentially. Maternal medical records were reviewed for indicators of maternal infection. Histologic chorioamnionitis was significantly associated with the usage of antibiotics (p = 0.0095) and a higher mean white blood cell count (p = 0.018). The presence of 1 or more clinical indicators was significantly associated with the presence of histologic chorioamnionitis (p = 0.019).

\\~\\
\textbf{Question}
\\~\\
Does histologic chorioamnionitis correspond to clinical chorioamnionitis?

\\~\\
\textbf{Yes}/No/Maybe

\\~\\
\hrule

\hypertarget{bioasq}{\section{BioASQ Example Question}}
\label{app:bioasq}

\\~\\
\\~\\
\\~\\
\hrule

\\~\\
\\~\\
\textbf{Context}

\\~\\
NT-pro-BNP was significantly elevated postexercise in both adults and adolescents and remained above baseline at 24 h in both groups. NT-pro-BNP concentrations increased significantly (28 +/- 17.1 vs 795 +/- 823 ng x L, P < 0.05), whereas postrace cTnT were elevated in just five athletes (20\%). [NT-pro-BNP] was observed immediately after the marathon (median [NT-pro-BNP] before: 39.6 pg ml(-1), after: 138.6 pg ml(-1), p=0.003) with a further increase on day one. [BNP] did not increase immediately after the marathon but increased on day one (median [BNP] before: 15 pg ml(-1), day one: 27.35 pg ml(-1), p=0.006). Pro-BNP was significantly increased immediately post-race (27+/-21 vs 7+/-2 pmol/L pre-race, P < or = 0.007), which 12-24 h later, decreased to 19+/-14 pmol/L (P = 0.07 vs pre-race). The relatively high NT-proBNP levels after active recovery when psychophysical stress is higher, because of cycling and cold water immersion, suggest that not only endurance exercise, but also strenuous, stressful short exercise can induce an increase in NT-proBNP concentrations. Running a marathon significantly increases NT-pro-BNP levels in healthy adults. This increase could be partially attributed to cardiac stress. Increases in NT-proBNP can be found in a major part of obviously healthy athletes after prolonged strenuous exercise. The release of BNP during and after exercise may not result from myocardial damage but may have cytoprotective and growth-regulating effects. The different nature of exercise-induced increases in BNP and cardiac troponins has to be elucidated in the future. In healthy cyclists, transient increases in NT-pro-BNP and cTnT are more likely to reflect cardiac fatigue than injury. The rise in BNP in older athletes may reflect a reversible, mainly diastolic left ventricular dysfunction.  Plasma BNP concentrations were higher in both the judo and marathon groups than in controls, and positively correlated with LV mass as well as with deceleration time. Such exercise significantly increased ANP and BNP levels in healthy men, and the increases could be partially attributed to myocardial damage during the race.

\\~\\
\textbf{Question}

\\~\\
Does BNP increase after intensive exercise in athletes?

\\~\\
\textbf{Yes}/No

\\~\\
\hrule

\\~\\
